TimeGPT-1

In this paper, we introduce TimeGPT, the first foundation model for time series, capable of generating accurate predictions for diverse datasets not seen during training. We evaluate our pre-trained model against established statistical, machine learning, and deep learning methods, demonstrating that TimeGPT zero-shot inference excels in performance, efficiency, and simplicity. Our study provides compelling evidence that insights from other domains of artificial intelligence can be effectively applied to time series analysis. We conclude that large-scale time series models offer an exciting opportunity to democratize access to precise predictions and reduce uncertainty by leveraging the capabilities of contemporary advancements in deep learning.

==> sections/conclusion.tex <==
\section{Conclusion} \label{section:conclusion}

- Potential use cases: fast inference, expert agnostic/limited human resources?

\MM{We believe the conclusions shown in the paper should deeply influence our thoughts around deep learning and time series. Particularly, we think our efforts merely show the potential for future developments.}

==> sections/dump.tex <==


\subsection{OLD}

We are constnalty faced with unceatainty. And we, as humans, try to reduce that incertanty all the time. From the ancient Greeks and Mayans, to the current research teams in Australia, China and USA some of the birghtest minds have been trying to find systemathic approaches to estimating the distribution of possible future events. 

Since the beginning of human history, in what can be considered the dawn of scientific thinking, people have been trying to estimate future uncertainty. At the heart of our discipline lies the desire to accrual predict possible outcomes and plan accordingly. 

Examples:
- Economic cycles, trends and seasonalities
- consumption patterns of buyers
- demand patterns of energy for production and grid optimzation
- capacity and infrastrucurte allocation for servers, workers, machines


Foundation models, with their ability to learn a broad range of tasks, have opened a new frontier in the field of artificial intelligence. Leveraging large-scale datasets, these models offer the potential to advance various sectors, from natural language processing to computer vision. This paper explores a new frontier in foundation models - their application to forecasting and anomaly detections through a new general model for time series: \ours.

While humans speak in time series, institutions, and systems rather use time series to represent their internal workings. Examples of time series are heights of ocean tides, counts of sunspots, and the daily closing value of the Dow Jones Industrial Average.

Time series analysis is pivotal in many domains, such as finance, health care, meteorology, and social sciences.  It involves deciphering temporal patterns, trends, and cyclical variations in data sequences ordered in time to forecast future values. These forecasts can significantly influence decision-making processes across various fields, from predicting stock market movements to anticipating patient health trends.

In the context of statistics, econometrics, quantitative finance, seismology, meteorology, and geophysics the primary goal of time series analysis is forecasting. In the context of signal processing, control engineering and communication engineering it is used for signal detection. Other applications are in data mining, pattern recognition and machine learning, where time series analysis can be used for clustering,[2][3] classification,[4] query by content,[5] anomaly detection as well as forecasting.[6]

\section{dump}

Historically, statistical methods have been extensively utilized in different domains. Examples include autoregressive integrated moving average (ARIMA) models and exponential smoothing. However, these methods often grapple with adequately capturing complex dependencies and non-linear relationships inherent in the data. They also struggle with scalability issues and require extensive feature engineering, which often necessitates domain-specific knowledge and does not guarantee optimal performance.


==> sections/ideas.tex <==

\MM{Additionally, more work should be done toward understanding trust in specific intuitions and models. metodologia pasada, arima 11, 2. habilidades visuales de juzgar algo, 3. la prediction no corresponds con nuestras expectativas. 4. selection adecuada de metrica de error, como Tim y Jan.}



It is known that the efficacy or success of metrics of a forecasting model is not always the average deviation metrics, but rather to particular process optimize.

Currently, there are no clear success criteria for a forecasting foundation model. Different domains might not only differ in the characteristics of the generating process measured by the time series but also in their assessment of the quality of the predictions. For instance, Physicians, traders, and retailers evaluate forecasting performance differently. This contrasts with the recent case of NLP foundation models, where success tests were devised by subjecting models to well-known exams. In other words, a successful model in NLP is, for most people, indistinguishable from humans, even for complex tasks like medical diagnosis.

In comparison, is not clear how one could test the general success of a forecasting foundation model, given the heterogeneous metrics for each task. 
A general model that was trained to minimize MAE might not be the best model when considering accounting for the success criteria of particular domains or tasks. \MM{esto es otra idea, limitation mas que debraye}

Figure \ref{fig:boxplot} presents the distribution of the rMAE per time series in the test set. \MM{Queres poner algo de esto?}


\begin{figure*}[t] %
\centering
\includegraphics[width=\linewidth]{images/correlations.pdf}
\caption{Error correlations}
\label{fig:correlations}
\end{figure*}



PAPERS

FROM TIM:

In the overall literature on forecasting, conclusive evidence of outsized gains in predictive accuracy of transformer-based
models is not yet available. On the one hand, results on publicly available data sets are positive [29], but not as
overwhelmingly positive as in natural language processing (NLP) where transformers dominate. Careful comparisons
with strong baselines (e.g., [7, 45]) place additional scrutiny on these results. We remark that transformer-based
forecasting approaches tend to distinguish themselves by side-aspects such as long-term forecasting or interpretability
whereas in NLP, the improvements in the core task are outsized.
On the other hand, on closed data sets, convincing evidence exists for the superiority of transformer-based forecasting
models, e.g., [12, 52]. Our results above point into a similar direction. So, a natural question to ask is whether (and
how) the success of transformer-based models can be associated to the nature of these closed source data sets and in
particular the abundace of data available for companies like Zalando. To make progress in answering this question, we
considered an often-cited reason for the success of transformers, so-called scaling laws (e.g., [23, 9]). These scaling
laws state that the predictive performance on a test set continues to increase for transformers along various dimension
including, for example, the size of the training set.
Concretely, we attempt to replicate scaling laws for transformers in forecasting, e.g., in [23, Figure 1] and whether we
can observe level effects (see Figure 11).








Concrete problems:
* exogenous
* multivariate
* arquitectures


- Limitations and future work:
\begin{itemize}
    \item exogenas, multivariate forecasting.
    \item Contextual knowledge of the underlying process generating the time series to improve accuracy
    \item Other time series tasks, like classification.
    \item Multimodality with other models/type of data like NLP and CV.
    \item How to judge a foundational model. Aggregate, individual series. Perdida how to train/optimize model. how to correlate with output.
    \item - Similitud entre series.
    \item - - Optimal setting the sclaing laws, is more data needed? What is the limit?
\end{itemize}




.\footnote{We sustain that this is also the case for the proposed taxonomy proposed by \citep{januschowski2020criteria} } 
}



We believe the polemic

\textcolor{red}{We believe that \ours\ takes a major step towards bringing these methods together under one unified approach} \MM{sacaria esto o hay que parafrasearlo}.

\CC{\ours\ combines the best}


ESRO PUEDE IMPORTAR!!!
OJO

A key facet of \ours\ is its commitment to democratization and accessibility, aiming to extend the benefits of advanced time series forecasting to a wider audience. 

To achieve this, \ours\ is designed to be modular and easily interfaceable, simplifying the integration into various systems and use cases. The goal is to minimize the complexity usually associated with implementing advanced forecasting models, encouraging widespread adoption. 

By offering user-friendly APIs, \ours\ further lowers the barriers to entry, enabling even those with limited technical expertise to harness the power of advanced time series forecasting. This encapsulation of complex systems into a digestible and approachable framework epitomizes the ethos of \ours: complex capabilities made accessible. \MM{Relocate in discussion. Podemos poner en esta section las ventajas generals de un Foundation model, como rapidez y democratization}
